Streamable Neural Audio Synthesis With Non-Causal Convolutions

Deep learning models are mostly used in an offline inference fashion. However, this strongly limits the use of these models inside audio generation setups, as most creative workflows are based on real-time digital signal processing. Although approaches based on recurrent networks can be naturally adapted to this buffer-based computation, the use of convolutions still poses some serious challenges. To tackle this issue, the use of causal streaming convolutions have been proposed. However, this requires specific complexified training and can impact the resulting audio quality. In this paper, we introduce a new method allowing to produce non-causal streaming models. This allows to make any convolutional model compatible with real-time buffer-based processing. As our method is based on a post-training reconfiguration of the model, we show that it is able to transform models trained without causal constraints into a streaming model. We show how our method can be adapted to fit complex architectures with parallel branches. To evaluate our method, we apply it on the recent RAVE model, which provides high-quality real-time audio synthesis. We test our approach on multiple music and speech datasets and show that it is faster than overlap-add methods, while having no impact on the generation quality. Finally, we introduce two open-source implementation of our work as Max/MSP and PureData externals, and as a VST audio plugin. This allows to endow traditional digital audio workstation with real-time neural audio synthesis on a laptop CPU.

==> body_ori.tex <==

\begin{abstract}
    %problem declaration
    %why problem is a problem
    %essence of the contribution
    %consequences of the previous point
    neural audio synthesis inside classical processing chain. audio deep learning inference is often performed on a request / response basis, either using cloud based services or directly on hardware. however classical dsp implies the processing of audio signals buffer-by-buffer, where the full context of the audio signal is not available. While existing approach relying on recurrent neural networks have successfully been ported to buffer-by-buffer computation, it is not the case for convolutional neural networks. In this paper we propose a way to build cnn that makes them compatible with buffer-by-buffer computations. We apply it to the recently proposed RAVE model and release the first cnn model compatible with real-time usage inside a classical audio software.
\end{abstract}


\section{Introduction}
%The introduction is where you tell the reader exactly the focus of the article. It should contain the purpose of the work, the problem and your approach. Explicitly declare the essence of your contribution.
% neural signal processing has set new sota in many fields. available for inference as cloud based services or as render engines. works for offline apps, however most of classical audio processing is performed on live streams.

Neural audio signal processing has set a new state of art in many fields, from audio source separation and text-to-speech systems to timbre transfer and unconditional generation. usually leveraging convolutional neural networks \cite{Lecun1995ConvolutionalTime-series} to build highly efficient models.
Early work on neural audio processing involved slower-than real-time synthesis procedures \cite{Oord2016WaveNet:Audio, Mehri2017Samplernn:Model, Vasquez2019MelNet:Domain, Wang2017Tacotron:Synthesis}, however the advent of adversarial learning \cite{Goodfellow2014GenerativeNetworks}, normalizing flow \cite{Rezende2015VariationalFlows} or diffusion models \cite{Ho2020DenoisingModels} have paved the way toward faster than real-time neural audio synthesis \cite{VanDenOord2018ParallelSynthesis, Kumar2019MelGAN:Synthesis, Prenger2019Waveglow:Synthesis, Chen2020WaveGrad:Generation}.
% should at some point define how live audio processing is performed, i.e using audio buffers.
While theoretically compatible with live audio processing (i.e processing live audio streams instead of previously recorded audio files), only a handful of models have been successfully ported to real-time audio applications (e.g the recently proposed DDSP model \cite{Engel2019DDSP:Processing}), and none of them are using convolutional layers but rather are based on recurrent neural networks.
Recurrent model can easily be ported to live streams processing by caching the recurrent state in-between DSP calls, and hence are a target of choice when addressing the deep learning based real-time audio processing task. On the other hand, processing live audio streams with a convolutional neural network is far from trivial, since the receptive field of the model is often far bigger than the audio buffer it is applied to.
Furthermore, processing two separate audio buffers using a convolutional neural network and then concatenating them results in clearly audible waveform discontinuities (e.g clicks), which are not acceptable for most audio applications. One possible solution for both problems would be to process large overlapping chunks of audio and cross fading them to smooth out hearable discontinuities, at the expense of a higher computational complexity, high latency processing, and degraded synthesis quality during transitional phases.

In this article, we propose a method to make convolutional neural network usable on live audio streams, without any approximation nor increase in computational complexity during synthesis. We achieve this by extending the cache operation proposed in \cite{Paine2016FastAlgorithm} to non-autoregressive networks and by re-arranging padding inside convolutional layers post-training to prevent it from relying on future audio samples during generation.
We also consider the case of parallel computation branches (e.g residual networks, skip connections) where additional delays are required for proper branch alignment.
We then apply our method to the recently proposed RAVE model \cite{Caillon2021RAVE:Synthesis} for comparison purposes against several baselines. We show how rearranging the padding pre-training significantly reduces the latency between model input and output to less than 30 ms when used on live audio streams.
We finally present several plugins that we developed in order to interface deep learning models with regular digital audio workstations, effectively presenting the first ever convolutional deep generative model applied in real-time on live audio streams, featuring 44.1kHz CPU synthesis and low-latency processing.



% specific architectures allow the processing of realtime streams (DDSP \cite{Engel2019DDSP:Processing}).
% ai speech denoiser performs in realtime. Based on RNN due to their simple implementation for buffer-by-buffer apps, but limits the amount of stuff we can do (most of the SOTA is convolutional).
% overlap-add can be used to use any kind of model work on live stream of audio at the expense of a higher memory and CPU consumption, latency and degraded audio quality

% we make CNN usable on live audio streams without approximation. rearrange padding to prevent model from seeing into the future. cache mechanism to resume computation between split buffers. branch alignment for residual blocks and architecture specific precautions.

% we first present our mechanism for real-time use of CNNs, then apply it to the RAVE model \cite{Caillon2021RAVE:Synthesis} in order to perform benchmarks and comparison with baselines, and finally present our developed apps.



\section{Method}
\label{sec:method}

Digital processing of an analog audio signal requires its discretization using an analog-to-digital converter, producing a digital stream with a sampling rate and resolution large enough to preserve information relevant to the human ear.
While some latency-critical applications require the processing of this stream one sample at a time, it is rather common to pack a number of samples into a buffer for later processing, increasing the processing latency while decreasing the processor load.

Convolutional layers process data with variable size by convoluting a learnable kernel over an input tensor. The kernel size, its dilation and the stride of the convolution altogether define the \textit{receptive field} of the layer (i.e the area around a particular location in the input tensor that is needed to produce an output). Stacking layers on top of each other increases the receptive field of the entire model, allowing the modelling of larger temporal dependencies \cite{Oord2016WaveNet:Audio}. It is however a problem for live audio streams since the processing of an audio buffer requires both past and future context, and can't be achieved knowing only the current buffered audio samples.



% convolutional neural networks process data with variable size. a kernel is convoluted over a tensor, the size of the kernel defines the receptive field of that particular layer. adding layers increases the receptive field. this causes two problems: receptive field sees in the future: not possible when working with live feeds. live audio stream are processed buffer by buffer, which is not trivial for CNN.

\begin{figure*}[ht]
    \centering
    \includegraphics[width=.75\linewidth]{img/convolution_cache.pdf}
    \caption{Convolution applied on two split buffers using cached padding. The last $\mathbf N$ frames from input buffer 1 are cached and concatenated with the input buffer 2 (with $\mathbf N$ being the original amount of zero padding) in order to prevent discontinuities between buffers.}
    \label{fig:cached_convolution}
\end{figure*}

\subsection{Processing buffers}

In order to maintain predictable tensor shapes, convolutional layers are often used in combination with \textit{padding}, which is a method to artificially increase a tensor shape in order to account for the receptive field of the model.
The padding mode \textit{center} consists in applying the same amount of padding at each end of a tensor particular dimension, as shown in Figure (\ref{fig:regular_padding}), effectively making the output of the convolutional layer "centered" with its input.
We call the padding at the left-side (resp. right-side) of the tensor \textit{pad L} (resp. \textit{pad R}) or \textit{left-padding} (resp. \textit{right-padding}). Left-padding is responsible for the need of a past context when processing an audio sample, whereas right-padding makes the model rely on future audio samples.

% Using convolutions that have a kernel size larger than 1 implies to take into consideration past and / or future context when processing an audio sample. to maintain coherent tensor shapes, convolutions are often use in combination with zero padding, as shown in figure \ref{fig:regular_padding}. left padding the tensor imply considering the past while right padding imply considering the future.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{.75\linewidth}
        \vskip 0pt
        \includegraphics[width=\linewidth]{img/convolution.pdf}
        \caption{Regular "center" padding, used during training}
        \label{fig:regular_padding}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.75\linewidth}
        \vskip 0pt
        \includegraphics[width=\linewidth]{img/convolution_causal.pdf}
        \caption{Re-arranged "causal" padding, used during inference}
        \label{fig:rearranged_padding}   
    \end{subfigure}
    \caption{Comparison between convolutions using regular padding and re-arranged padding. Using re-arranged padding we implicitly delay the input in order to get the required overhead.}
    \label{fig:convolutions}
\end{figure}

When processing live audio streams, using future samples can be achieved by introducing latency in the processing chain in order to get the required overhead.
We implement this by re-arranging padding for each convolutional layers after training, replacing right-padding with left-padding, as shown in Figure (\ref{fig:rearranged_padding}). Using this re-arranged padding, we keep the same tensor shapes while taking into account only past and present samples.

Processing two separate buffers and concatenating the output results in audible discontinuities caused by the introduction of padding in between each buffer. We therefore replace the aforementioned zero padding with \textit{cached} padding, where we keep in memory the last $N$ samples from a tensor and use it to left-pad the next one, as demonstrated on Figure (\ref{fig:cached_convolution}). This cached padding method can be seen as an extension of the one proposed in \cite{Paine2016FastAlgorithm} to buffer-based neural audio processing. Using this mechanism we can "resume" the convolution operation from one buffer to another, addressing the previously mentioned audio discontinuities (see Section \ref{sec:audio-quality} for an ablation study).



\subsection{Synchronizing parallel branches}

The aforementioned cached padding mechanism is sufficient to make simple convolutional neural networks operate on live streams, however models with parallel computation branches (e.g residual layers or skip connections) need an extra level of attention. In fact, if the receptive field of each parallel branch is not equal, the delay induced by re-arranging padding results in misaligned outputs for each branch, making the model behave unpredictably. It is therefore crucial to keep track of those parallel branches and introduce compensatory delays where needed to properly align each branch with relation to each other, as demonstrated in Figure (\ref{fig:alignment}). 

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{.49\linewidth}
        \vskip 0pt
        \includegraphics[width=\linewidth]{img/alignment_training.pdf}
        \caption{during training}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\linewidth} 
        \vskip 0pt
        \includegraphics[width=\linewidth]{img/alignment_inference.pdf}
        \caption{during inference}
    \end{subfigure}
    \caption{Aligning a residual connection for real-time inference. Re-arranging padding for real-time inference implies a delay that must be applied to every other parallel branches for proper output alignment.}
    \label{fig:alignment}
\end{figure}



\subsection{Architecture specific alignment}

rearranged padding shifts the way the model is built. for most classical architectures cache + alignment is enough. but for weird combination such as conv transpose followed by stride conv it is not enough and proper synchronization must be applied.

another weird case is when you have parallel branches that compress / expand the tensor temporal dimension. in this particular case we must be careful to apply the delay where on the larger tensor (after conv for upsampling, before conv for downsampling).

\section{Experiments}
\subsection{RAVE}

The RAVE model \cite{Caillon2021RAVE:Synthesis} is a Variational Auto Encoder \cite{Kingma2014Auto-encodingBayes} aiming at generating high-quality 48kHz audio signals. It leverages a multiband decomposition of the raw waveform as a way to decrease the temporal complexity of the waveform, allowing 20 to 80 times faster than real-time neural audio synthesis on a standard laptop CPU. RAVE is a feed forward model, composed of an encoder (a regular strided convolutional network), and a decoder (a residual transposed convolutional network). Its overall architectural simplicity and synthesis quality make it a good candidate for experiments on the adaptation of deep convolutional models to live audio stream processing.

\subsection{Baselines}
\label{sec:baselines}

We compare our method presented in Section \ref{sec:method} against the following baselines.

\subsubsection{Offline reconstruction}
We compare all methods against the regular \textit{offline reconstruction} procedure of the model, where we reconstruct a pre-recorded audio signal all at once, setting an upper bound to the generation quality.

\subsubsection{Simple buffer-based}
The first baseline we implement is the \textit{simple buffer-based} method, ignoring the issues reported in Section \ref{sec:method} and applying the unmodified model directly on live audio streams, processing buffers one by one and concatenating the outputs prior to listening to the result.

\subsubsection{Overlap-add}
A convenient way to avoid harsh discontinuities between buffers is the \textit{overlap-add} method. We implement this method by caching a large chunk of audio (i.e large enough to account for the receptive field of the model), and process it the same way offline processing is performed. We then window the resulting signal using 
%
$$
\mathbf w[n] = \sin \left ( \frac{\pi n}{N} \right )^2,
$$
%
where $N$ is the chunk size. We finally overlap-add the resulting tensor over the previous output signal with a hop length of $N$.


\subsection{Addressing model latency}
\label{sec:addressing_latency}

% Re-arranging padding to strictly causal post-training implicitly adds latency to the model. We show that re-arranging padding pre-training leads to significantly reduced latency see figure \ref{fig:latency}. However, this re-arrangement makes the modelling task more difficult, resulting in a small drop in audio quality.

The post-training padding re-arrangement introduced in Section \ref{sec:method} is crucial to prevent the model from relying on future audio samples when operating in real-time, which inevitably adds some latency to the model (i.e the delay observable between the model input and output). Since the receptive field of the RAVE model extends up to 600ms into the future, this exact amount of delay will be heard when using this model in real-time, which can be a problem for latency critical applications. We therefore experiment with re-arranging padding \textit{prior} to the training, making the model learn to reconstruct audio samples in a causal fashion. This allow to drastically reduce the latency of the model from $\sim600$ms to $\sim 30$ms, as demonstrated in Figure \ref{fig:latency}. The remaining latency comes from the compression ratio of the model (i.e the full stride of the encoder) that makes it need a fixed amount of audio samples in order to produce a single latent point. Reducing latency even more can thus be achieved by reducing the compression ration of the model, which can have a negative impact on the performances of the model.

\begin{figure}[ht]
    \centering
    \includegraphics[width=.9\linewidth]{img/latency.pdf}
    \caption{Real-time reconstruction of a noise burst by two models trained on percussive sounds, one with post-training padding re-arranging (regular), the other with pre-training re-arranging (no latency).}
    \label{fig:latency}
\end{figure}

Unlike post-training padding rearrangement, training the model in this causal configuration makes the modelling task more complex and may result in decreased model performances.

\subsection{Datasets}

We evaluate the performances of our method using RAVE trained on three different datasets with different acoustic properties. We train RAVE twice for each dataset (pre-training padding rearrangement and regular training).

\subsubsection{Speech}

wheel: 9h20mn

\subsubsection{Darbouka}

darbouka: 2h33mn

\subsubsection{Koto}

koto: 3h23mn




\section{Results}
\subsection{Audio quality}
\label{sec:audio-quality}
We reconstruct a 2 second long audio sample using RAVE with the methods listed in \ref{sec:baselines}, and display their rainbowgrams in figure \ref{fig:comparison_rainbow}.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/rain_full.png}
        \caption{Offline rendering}
        \label{fig:rain_full}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/rain_naive.png}
        \caption{Simple buffer-based}
        \label{fig:rain_naive}
    \end{subfigure}
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/rain_ola.png}
        \caption{Overlap-add}
        \label{fig:rain_ola}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/rain_cache.png}
        \caption{\textbf{Our method}}
        \label{fig:rain_cache}
    \end{subfigure}
    \caption{Rainbowgrams \cite{Engel2017NeuralAutoencoders} of audio samples reconstructed using different methods (offline, simple, overlap-add, and our method), with a buffer size $2^{14}$.}
    \label{fig:comparison_rainbow}
\end{figure}

Using the naive method to generate sound yields clearly audible discontinuities, as shown in figure \ref{fig:rain_naive}. While the overlap-add method in figure \ref{fig:rain_ola} gets rid of those discontinuities, the cross-fade between contiguous buffers alters the phase and produce a noisy instantaneous frequency, perceptually producing a "blurry" sound. In comparison, the cache method in figure \ref{fig:rain_cache} behaves exactly like the full method, without any phase distortion or discontinuity. We quantitatively evaluate all methods by evaluating their similarity with the offline generation procedure, using the following distances
%
\begin{align}
    \nonumber \mathcal L_{s}(\mathbf x, \mathbf y) &= \| \log (S(\mathbf x)+\epsilon) - \log (S(\mathbf y)+\epsilon) \|_2 \\
    \mathcal L_{c}(\mathbf x, \mathbf y) &= \frac{\sum_n \mathbf x[n]\mathbf y[n]}{\sqrt{\sum_n \mathbf x[n]^2 \sum_n \mathbf y[n]^2}},
\end{align}
%
where $\mathcal L_s$ is a spectral distance between amplitude spectrograms $S(\cdot)$, and $\mathcal L_c$ is a normalized correlation score. We compensate the latency mentioned in Section \ref{sec:addressing_latency} prior to evaluating those distances, and report the results in Table \ref{tab:quantitative_results}.

\begin{table}[ht]
  \caption{\itshape Quantitative reconstruction evaluation}
	\centering
	\begin{tabular}{|c|c|c|}
		\hline Method & Spectral distance & Correlation\\\hline
		simple & 0.00 & 0.00 \\
		overlap-add & 0.00 & 0.00 \\
		\textbf{ours} & 0.00 & 0.00 \\\hline
	\end{tabular}
	%
	\label{tab:quantitative_results}
\end{table}

we also evaluate perceptually how those methods compare (offline, simple, ola, cache, cache nl) and report the results in Table \ref{tab:perceptual_results}.

\begin{table}[ht]
  \caption{\itshape Perceptual evaluation}
	\centering
	\begin{tabular}{|c|c|}
		\hline Method & MOS\\\hline
		simple & 0.00  \\
		overlap-add & 0.00  \\
		\textbf{cache} & 0.00 \\
		\textbf{cache nl} & 0.00 \\\hline
	\end{tabular}
	%
	\label{tab:perceptual_results}
\end{table}

\subsection{Performances}

Processing high-resolution images or long audio samples with deep convolutional models has a non-negligible cost in term of memory consumption and computation time. A system with a fixed amount of RAM will therefore be limited in terms of the maximum resolution or duration it can handle for a particular model, as demonstrated in Figure \ref{fig:full_benchmark}. 
% processing increasingly long audio samples using offline rendering leads to an increase in RAM consumption, potentially limiting the audio duration a given system can handle see figure \ref{fig:full_benchmark}.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/full_mem.pdf}
        \caption{Memory usage}
    \end{subfigure}
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/full_time.pdf}
        \caption{Computation time}
    \end{subfigure}
    \caption{Offline audio reconstruction benchmark using RAVE on increasingly long audio samples. In order to account for memory and time measurement errors, we average the two quantities over 10 trials.}
    \label{fig:full_benchmark}
\end{figure}

In contrast, processing audio using buffers results in a memory usage that only depends on the buffer size, and not the total duration of the audio signal. Models operating on buffers can consequently process arbitrary long audio samples, with a linearly increasing computation time. We compare on Figure \ref{fig:buffer_benchmark} the memory footprint and real-time factor of the \textit{overlap-add} and \textit{cache} methods for increasingly long buffer sizes, and demonstrate that the \textit{cache} method needs less memory and computation time than the \textit{overlap} method for identical buffer sizes. Furthermore, the \textit{overlap} method needs at least $\sim 2.5$s long buffers in order to fill the receptive field of the model in its entirety. On the contrary, the \textit{cache} method can use buffers as small as the compression ratio of the model, allowing the use of RAVE on arbitrary long audio signals using less than 50MiB of RAM.

% processing audio using buffers results in a memory usage only depending on the buffer size, while the total audio duration has no effect on it. we compare on figure \ref{fig:buffer_benchmark} the memory footprint of ola and cache for increasingly long buffer size. We demonstrate that cache has a lower memory footprint and real-time factor than ola, while allowing to use significantly lower buffer size.

\begin{figure}[ht]
    \centering
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/buffer_mem.pdf}
        \caption{Memory usage (lower is better)}
    \end{subfigure}
    \begin{subfigure}[b]{.49\linewidth}
        \includegraphics[width=\linewidth]{img/buffer_time.pdf}
        \caption{Real-time factor (lower is better)}
    \end{subfigure}
    \caption{Buffer based audio reconstruction benchmark using RAVE on increasingly long audio samples for two methods, overlap-add (ola) and our method (cache). Dotted lines indicate that the model is operating on buffers that are smaller than its receptive field, degrading its modelling abilities. In order to account for memory and time measurement errors, we average the two quantities over 10 trials.}
    \label{fig:buffer_benchmark}
\end{figure}


% We therefore show that using cached convolution we can obtain the exact same network behavior as offline rendering while keeping a low memory footprint (under 50MiB) by processing audio buffer by buffer, expending its use to live audio stream processing.


\subsection{Integration inside real-time frameworks}
is it appropriate to put that here ? 

We build several application to showcase the real-time use of such models
- max / msp (macOS + windows)
- puredata (linux)
- VST (macOS + windows)

Using a light weight RAVE we even show that we can obtain 48kHz unconditional generation in real-time on a non-overcloked raspberry Pi 4.


\section{Conclusion and Future Perspectives}
%This section must actually contain your conclusions about your results. It must be comprehensible even to someone who has not read the article and you should not reference new material that was not presented in the article

%Briefly restate the problem described in the introduction
%Declare whether the problem was completely solved
%Declare the limitations and implications of your contribution
%Present future perspectives of the work based on the conclusions above

usual deep learning apps work in an offline fashion when classical DSP operates on live audio streams. this make the use of DL models complex as it does not integrate well existing creative workflows. we propose a method to circumvent this problem and deploy dl models inside real-time framework using cached convolutions, causal padding and careful temporal alignment of parallel computation branches present inside the neural network. we apply our method to the RAVE model and therefore propose the first CNN model operating on live audio streams without any approximation compared to its offline version.



\bibliographystyle{unsrt}
\bibliography{references}

